A Survey on Self-Supervised Representation Learning

Learning meaningful representations is at the heart of many tasks in the field of modern machine learning. Recently, a lot of methods were introduced that allow learning of image representations without supervision. These representations can then be used in downstream tasks like classification or object detection. The quality of these representations is close to supervised learning, while no labeled images are needed. This survey paper provides a comprehensive review of these methods in a unified notation, points out similarities and differences of these methods, and proposes a taxonomy which sets these methods in relation to each other. Furthermore, our survey summarizes the most-recent experimental results reported in the literature in form of a meta-study. Our survey is intended as a starting point for researchers and practitioners who want to dive into the field of representation learning.

==> sections/memory.tex <==
\subsection{Memory Banks for Contrastive Learning} \label{sec:memory-bank}
Contrastive methods tend to require in optimization batches large amounts of
negative samples to learn a useful representation for downstream tasks
\citep{bardes2021vicreg}.

\todo{SW: Contrastive methods tend to require large amounts of negative samples
  in optimization batches to learn a useful representation for downstream tasks
  \citep{bardes2021vicreg}.}

So far, this number of encodings can not be efficiently computed and
parallelized which makes it costly to assemble these batches. The current
(non-optimal) solution is to save already computed encodings of images and reuse
them when they are queried, known as memory banks \citep{wu2018unsupervised}.
However, the representations in the memory bank can become outdated and need to
be periodically updated in order to maintain validity.\todo{SK: e.g. moving averages}

\paragraph{Hard negative mining with memory banks.}
Hard negative samples exhibit similar features to certain positive samples but
differ in their assigned classes. It is in our interest to find and insert these
hard samples in a batch to ensure a strong gradient signal
\citep{zhang2021understanding}. In contrastive learning, encountering only
easily identifiable negatives in a batch results in a vanishing gradient.
Increasing the batch or memory bank size leads to a higher probability to
encounter a hard negative sample but yields no guarantee. To further improve
this mechanism, novel hard negatives can be found by searching for adjacent data
points \citep{bulat2021improving} (e.g., K-NN on memory bank encodings). This
technique is applicable for supervised and self-supervised cases where there is
a clear separation between the positive and negative distribution.

